Using Inaudible Audio to Improve Indoor-Localization- and Proximity-Aware Intelligent Applications

While it is often critical for indoor-location- and proximity-aware applications to know whether a user is in a space or not (e.g., a specific room or office), a key challenge is that the difference between standing on one side or another of a doorway or wall is well within the error range of most RF-based approaches. In this work, we address this challenge by augmenting RF-based localization and proximity detection with active ultrasonic sensing, taking advantage of the limited propagation of sound waves. This simple and cost-effective approach can allow, for example, a Bluetooth smart-lock to discern whether a user is inside or outside their home in order to lock or unlock doors automatically. We describe a configurable architecture for our solution and present experiments that validate this approach but also demonstrate that different user behavior and application needs can impact system configuration decisions. Finally, we describe applications that could benefit from our solution and address privacy concerns.

==> Inaudible audio IUI/applications.tex <==
\section{Usage Scenarios}

We envision the use of our solution in a variety of different applications in two primary categories: controlling access to services and controlling access to spaces.

\subsection{Controlling access to services}
\emph{Secure document access.}\quad
Previous work has used precise indoor localization to ensure that users have access to certain sensitive documents (e.g., financial, medical) only while they are at a particular private location. This is often accomplished using GPS and Geofencing or similar techniques \cite{Doclock}. However, these techniques provide only coarsely-defined secure areas, allowing malignant parties to potentially access documents on the boundaries. Similarly, LocAssure \cite{biehl_youre_2015} proposed to provide assurances of a user's reported location, but their underlying system still depends on the accuracy of the (BLE) localization infrastructure. By comparison, our RF- and US-based approach can allow users to define much more fine-grained secure areas with much lower risk of adversarial document access.

\emph{Improved location-based notification.}\quad
Location-based reminders and notifications have been demonstrated in both outdoors \cite{sohn_placeits} and indoors \cite{lin_location-based_2012} settings. However, with the limited accuracy of RF-based localization, applications run the risk of delivering notifications at incorrect moments or miss otherwise useful opportunities. For example, due to the low accuracy of Bluetooth-based localization, Cambo \textit{et al.} \cite{cambo_breaksense:_2017} relied on changes in physical activity recognized by a smartwatch to trigger notification, which resulted in notification lag. Our solution would help ensure that location-based notifications arrive appropriately.

\subsection{Controlling access to space}
\emph{Smarter smart locks.}\quad
Current smart locks \cite{august,fridaylabs,ottoCNET,danalock} make use of Geofencing to automatically unlock the door when a user's device is in proximity of the lock. However, such locks will typically rely on several assumptions that can lead to errors.
For example, after automatically unlocking the door for the user, the system may incorrectly assume that the opening and then closing of the door means that the user is now inside the home when, in fact, they stayed outside, leading to an incorrect system state.
By adding our solution to the internal-facing plate of the smart lock, for example, the system will correctly sense whether the user has entered their home. Based on the results presented above, to support a phone carried in a bag or purse, the lock should be configured as a receiver.

\emph{Private, rentable workspaces.}\quad
``Workbooths'' such as Jabbrrbox \cite{jabbrrbox}, Zenbooth \cite{zenbooth}, and others, placed in public areas, allow users to schedule and pay to have a temporary, private workspace. Such rentable workspaces, which combine scheduling and access control, would benefit from correct knowledge of whether a specific user is inside or outside their scheduled space. 
The scheduling and access-control systems would be able to, for example, determine whether a user's scheduled time is active, granting them repeated access while preventing access from others (see Figure \ref{fig:human}). If multiple workspaces are located in close proximity (preventing RF-based localization from pinpointing a user's location), our solution's ability to broadcast encrypted, identifying messages through multiple ultrasonic channels would ensure that users have access only to the spaces they have scheduled.

\begin{figure}[tb]
\centering
\begin{tabular}{cc}
\includegraphics[width=1.5in]{figs/2.jpg} & \includegraphics[width=1.5in]{figs/3.jpg} \\
% \includegraphics[width=1.5in]{figs/3.jpg} & \includegraphics[width=1.5in]{figs/5.jpg} \\ \includegraphics[width=1.5in]{figs/1.jpg} & \includegraphics[width=1.5in]{figs/4.jpg} \\
\end{tabular}
\caption{Use-case illustration: Controlling access to private, rentable workspaces. A scheduling and access-control system uses inaudible audio to determine whether to grant access to a user at a particular time.}
\label{fig:human}
\end{figure}

==> Inaudible audio IUI/applications_leftovers.tex <==
% \subsection{Telemedicine kiosks}
% Most doctor visits are fast, taking only on average ~17 minutes \footnote{https://www.ncbi.nlm.nih.gov/pmc/articles/PMC2254573/}. However, it can be important for a doctor to have some basic information about a patient's medical history, such as test results or past and current prescriptions, before making a diagnosis. For visits at a traditional doctor's office, obtaining this information securely is straightforward. However, at a telemedicine kiosk this information would need to be sent from a patient through a wireless network, and nearby malingerers could intercept the data. Information could be encrypted on the user's mobile device, but in some cases that may take too long or be impractical. Sending information back-and-forth from the patient to the booth via ultrasonic communication, then relying on the booth system to encrypt and send the data to the doctor over a wired network, could provide a high level of security and privacy without forcing users to worry about encrypting their data.

% \subsection{Room-based music differentiation}
% While homes and workspaces often share a common music service (e.g., Sonos), people may want to play different music in different rooms or office spaces. While this is technically possible with such systems, since they have no method of determining the room a user is currently in, the process is complicated \footnote{ https://drive.google.com/file/d/1mI9AOixsZpxDrxVnsnzYQbPZ23bSV-EG/view}. Furthermore, these systems can be trivially hacked so that users in one part of the house or office play unwanted music in a different part of the house or office. 

% On the other hand, using a combination of mobile devices and IAX beacons, the system can be configured to play music in the current room and only the current room with a single button press. Furthermore, since IAX beacons can be any device with a speaker, an Alexa (or similar) device can be re-purposed as an IAX beacon. 

% \subsection{Conference presentations}

% \begin{figure}[htb]
% \centering
% \begin{tabular}{cc} 
% \includegraphics[width=1.5in]{figs/confUI1.png} & \includegraphics[width=1.5in]{figs/confUI2.png}\\
% \end{tabular}
% \caption{At many conferences, attendees can take advantage of mobile apps that provide special services for talks. Without IAX beacons (left), users must manually find the room they are currently in. With IAX beacons (right), their device can automatically find their current room and allow them to access services directly.}
% \label{fig:conference}
% \end{figure}

% Increasingly, conferences offer extra services to audience members, such as slides of the current talk or a backchannel chat or translation services \cite{lanbridge}. While, again, using Bluetooth or other EMF-based technologies would make it possible to select the current talk amongst a list, in large conferences with many simultaneous talks it would be difficult to find the one occurring in the room the user is in. On the other hand, using ultrasonic audio, the user can can connect directly to the talk happening in their room. Furthermore, speakers could include interactive sections of their talk, including live polling or feedback solicitation, and be confident that only those audience members currently in the room would be able to participate.

% In some environments, these technologies are therefore combined with motion senors, NFC or other very near-field technologies to determine actual presence in a space. However, motion sensors cannot attribute presence to a particular individual (or device) and near-field technologies require users to actively badge in to a room, which can be cumbersome or produce state errors if the user forgets to badge out.

% Our combined RF- and ultrasonic-based approach, on the other hand, can reduce or eliminate these ambiguities without requiring the user to take any explicit action. In this case, the Smart Lock would act as the receiver, listening to ultrasonic messages sent from the mobile on the inside of the door. Once it receiving messages from the interior ultrasonic sensor, and the door is shut, it can safely assume that the user is inside and lock the door.

% Contrary to EMF waves, sound waves are more likely to respect wall and door boundaries and therefore can be more useful for threshold boundary scenarios (Figures \ref{fig:waves} and \ref{fig:waves2}). Furthermore, unlike NFCs, they do not require any specific user actions. They can also send a small amount of data over short distances, providing extra information at a short range, which is not possible with NFC.

% Private workbooths, such as Jabbrrbox \cite{jabbrrbox}, that are placed in public areas rely on automatic access systems that our RF- and ultrasonic-based approach can augment. Here again, the system can use an RF sensor coupled with an internal ultrasonic receiver to determine whether the user is outside or inside the workbooth. Furthermore, the system can connect to an external service that indicates whether the user currently has access to a nearby workbooth, allowing the system to determine the following several states. 

%\begin{figure}[tb]
%\centering
%\includegraphics[width=2in]{figs/jabbrrbox.jpg} 
%\caption{The Jabbrbox workbooth  \cite{jabbrrbox}.}
%\label{fig:jabbrrbox}
%\end{figure}

% \textbf{Session active, user is away from both the RF and US beacons:} The system notifies the user to proceed to the workbooth. 

% \textbf{Session active, the workbooth detects that the user is in RF range (only):} The system unlocks the door for the user.

% \textbf{Session active, the workbooth detects that the user in US range and the door is shut:} The system locks the workbooth. 

% \textbf{Session inactive, the workbooth detects that the user in US range:} The system unlocks the door for the user and notifies the user that their session is over. 

% \textbf{Session inactive, the workbooth detects that the user is not in US range:} The system takes no action. 

% The default case is that the system will remain locked. 

% One additional useful case is when several workbooths are located next to one another in the same space. In this case, the system can broadcast encrypted, identifying messages on unique RF and US channels to provide the user access only to the workbooth they have scheduled.



==> Inaudible audio IUI/conclusions.tex <==

\section{Conclusions}
We presented a simple and cost-effective solution for helping RF-based localization and proximity systems overcome the challenge of determining positions near thresholds such as walls and doors. Our approach takes advantage of the limited propagation of sound waves between enclosed spaces. Our evaluation showed high performance of the solution, especially when the user's phone is held or in a pocket. Finally, we discussed performance and privacy trade-offs that must be considered based on the intended target application.



==> Inaudible audio IUI/discussion.tex <==

\section{Discussion}
The evaluation demonstrated the viability of using ultrasonic audio as a low-cost solution to determine whether a user is on one side of a threshold or another---important for location- and proximity-aware smart applications. 
Performance when the phone was in a bag was lower. For this reason, in future work we plan to implement and evaluate our solution using a smartwatch, since it is less likely to be obstructed.

The evaluation also highlighted an important trade-off when deploying this solution. Specifically, in order to support detection when the user carries their phone in a bag (i.e., avoid false negatives), our tests suggest that the phone needs to be configured as a beacon and fixed devices as receivers. However, the tests also show that when the door is open and a phone, configured as a beacon, is held in hand, messages are more likely to be incorrectly received from the other space (false positives). While in some cases this trade-off could be resolved through simple door-state sensing (e.g., magnetic sensors), we demonstrate that the configuration of beacons and receivers should be considered based on the application to optimize for fewer false positives or false negatives. 

Finally, a critical area for location-aware applications in general, and for applications that rely on acoustic sensing in particular, is the threat to users' privacy (\textit{cf.}, \cite{chitkara_does_2017,klasnja_exploring_2009}). Indeed, in addition to performance trade-offs, the two configurations of our solution may have different implications for privacy. In the first configuration,  the mobile phone's microphone is opened once in RF range of a beacon, listening for ultrasonic phrases. This requires the user to grant the application access to the phone's microphone---something users may be hesitant to do. Still, a key benefit of using the phone as a receiver is that sensing can be performed locally on the phone without disclosing information about the user.
The second configuration, on the other hand, requires stationary microphones to be present and listening in the environment. Through the promise of only listening to ``wake words'', stationary, always-listening devices such as Amazon Alexa Echo \cite{noauthor_amazon_2015} and Google Home \cite{noauthor_google_2016} have become commonplace in recent years, suggesting that users may be comfortable with this configuration (although research has shown various possible risks associated with these devices \cite{arp_privacy_2017}). Always-listening devices are, however, only beginning to find acceptance in workplace environments \cite{alexa_for_business}. We argue that considerations of privacy and performance must both be taken into account when implementing and deploying solutions such as the one described in this paper.

==> Inaudible audio IUI/eval_leftovers.tex <==


% \paragraph{Inaudible audio is secure} In all cases in which the door was shut and the user location was different from the fixed device location (1040 total samples), zero messages were transferred. This implies that if a user is outside of a room with the door shut the system will never erroneously register a user as inside a room. However, in further experimentation, we found that this is only true if the door is well insulated (that is, a user holding a device right next to a poorly insulated closed door may be able to send messages to an interior fixed device). 

% \paragraph{Message sending works well when the device is unimpeded but degrades rapidly} When the user is on the same side as the fixture location and holding the device in their hand, message sending works well (320/320 received in the near condition, 311/320 received in the far condition). Also, a relatively high percentage of messages are received when the device is in a user's pocket (301/320 received in the near condition, 178/320 received in the far condition). However, far fewer messages are received when the device is placed in a bag (79/320 received in the near condition, 9/320 received in the far condition). While not surprising, this result does imply that users who tend to carry their device in a bag or purse will need to take it out or rely a smartwatch. 

% \paragraph{Messages sent from the mobile are more likely to be received than those sent from a fixed device} More messages are transferred when the mobile device is the one sending data (814/1920 events received by the fixed device) than the reverse (555/1920 events received by the mobile). This is especially true when the mobile device is in a bag and sending (82/640 events received at the fixed location) versus receiving (6/640 events received by the mobile). This implies that the device's microphone suffers more attenuation than does its speaker.

% \paragraph{It is possible to detect when the door is open in some cases} When the user is on the opposite side from the fixed device, near the threshold, and the user is holding the device in their hand, the system can potentially detect that the door is open (107/320 events received) versus shut (0/320 events received). However, if the device is in a user's pocket, the difference between open (41/320 events received) and shut (0/320 events received) is smaller. The difference between the door being open and shut is not detectable when the device is in a bag (0/320 for both cases).

%\colorbox{pink}{highlight}

%%To better understand the performance of our solution under a range of conditions, we carried a set of experiments.

%%We compared:

%%Door type
%%Indoor vs. Outdoor performance
%%Mobile device location (in hand vs. pocket vs. purse)

%%We tested each combination at four positions as illustrated in Figure XXX; two positions outside and two positions inside. We further tested each combination with the door open and with the door shut.

%%Test devices:  Android? Google Pixel vX?
%%Based on a pilot test, transmission volume in all tests was set to XXX. 

%%In each test case, the system transmitted the phrase 20 times. Our recognition results are presented as a percent of phrases picked up correctly by the receiving device.

==> Inaudible audio IUI/evaluation.tex <==
\section{Evaluation}

% Replace pocket photo for camera ready
\begin{figure}[tb]
\centering
\begin{tabular}{cccccc} 
\multicolumn{3}{c}{\includegraphics[width=1.5in]{figs/office_shut_in.jpg}} & \multicolumn{3}{c}{\includegraphics[width=1.5in]{figs/home_closed_out_tweaked.jpg}} \\
\multicolumn{2}{c}{\includegraphics[width=.95in]{figs/phoneHand.jpg}} & \multicolumn{2}{c}{\includegraphics[width=.95in]{figs/phonePocket.jpg}} & 
\multicolumn{2}{c}{\includegraphics[width=.95in]{figs/bag.jpg}}
\end{tabular}
\caption{We evaluated the system in different environments (top) and contexts, with the mobile device held in hand, in a pocket, or placed in a bag (bottom).}
\label{fig:eval}
\end{figure}

We evaluated effectiveness of our approach for detecting a user's position relative to a threshold, examining a range of conditions, including different device contexts and threshold types. We tested the following conditions:

\textbf{Environment} (2): We compared performance for a \emph{home} entryway and an internal \emph{office} door (Figure \ref{fig:eval}, top).

\textbf{Door state} (2): While intended to work when a space is enclosed, we tested with doors both \emph{shut} and \emph{open}.

\textbf{Fixed device location} (2): A fixed device (Figure \ref{fig:eval}, top) is either \emph{internal} or \emph{external} (e.g., in the office vs. hallway).

\textbf{User location} (2): The user was in the \emph{same space} as the fixed device or in the \emph{other space}.

\textbf{Distance} (3): The user was \emph{10 ft}, \emph{2 ft}, or \emph{0 ft} from the threshold. We tested the  \emph{0 ft} distance only with the door shut and on the other side from the fixed device.

\textbf{Mobile Context} (3): The mobile was held in \emph{hand}, in a \emph{pocket}, or in a standard canvas \emph{bag} (i.e., purse). (Figure \ref{fig:eval}, bottom)

\textbf{Configuration} (2): The mobile acted as a beacon (\emph{mobile beacon}) or a receiver (\emph{mobile receiver}).

\subsection{Setup}
We performed tests using two Google Pixel (v1) devices, one fixed and mounted next to the door near its handle (see Figure \ref{fig:eval}) and one mobile. We set the volume level of both devices as high as possible such that no audible artifacts were detected (for the devices used, this was volume level 11/15). In each test, the beacon application sent a simple hexadecimal message (``0xaa'') 20 times, and the number of messages ``heard'' by the receiving device is reported. We collected a total of 4,320 samples (20 samples x 216 condition-combinations).

% We also ran an additional set of 24 tasks simulating a situation in which someone on the one side of a threshold was attempting to appear as if they were actually on the other side (e.g., we moved the mobile device as close as possible in \emph{hand}, \emph{pocket}, and a \emph{bag} next to a closed door in both the \emph{office} and \emph{home} settings and with the beacon originating from both the \emph{mobile} and \emph{fixed} devices with the user \emph{inside} and \emph{outside} and the fixed device on the opposite side of the user). All told, we collected 4320 samples (216 conditions * 20 samples per condition).

\subsection{Results}

\begin{figure}[t]
\centering
\begin{tabular}{c} 
\includegraphics[width=3.25in]{figs/Graph1bw.png}
\end{tabular}
\caption{Percent of messages received at different distances (in feet) from a closed door. in different usage contexts with the mobile device configured as a \emph{beacon} (top) and \emph{receiver} (bottom). In the ideal case, no messages are received from the other space (left side), and 100\% of messages are received in the same space (right side). }
\label{fig:results}
\end{figure}

\begin{figure}[t]
\centering
\begin{tabular}{c} 
\includegraphics[width=3.35in]{figs/Graph2bw.png}
\end{tabular}
\caption{Percent messages received for the door shut and door open conditions when the device shares the same space as the fixed device versus the other space. Illustrates how, with the door open, messages leak from the other space.}
\label{fig:results_door}
\end{figure}

Figure \ref{fig:results} shows the percent of messages received at different distances from a closed door, in different usage contexts (hand, pocket, and bag), when the phone is configured as a beacon (top) or a receiver (bottom). 
The results show that our approach works well, particularly when the phone is in the user's hand or pocket. 87\% of messages (1110 of 1280) were correctly received from a beacon in the \emph{same space} and, importantly, when the door is shut, not a single message was incorrectly received from a beacon in the other space (0/1440). In other words, when the door is shut, our system produces no false positives. We should note, however, that when the phone is inside a bag, performance is only adequate when standing near the door and the phone is configured as a beacon. 
There was no significant difference in performance between the office and home environments.

As can be seen in Figure \ref{fig:results_door} left, our system is able to distinguish extremely well standing next to, but on opposite sides of a closed door---our key use-case. However, not surprisingly, when standing near an open door (Figure \ref{fig:results_door} right), the system picks up inaudible messages from the other space (in our tests, 171 of 640 messages, or 27\%), particularly when the phone is held in the user's hand and is configured as a beacon.

Finally, we observed that more messages were received when the mobile device acted as a beacon (\emph{mobile beacon}) than as a receiver. 
As mentioned above, when placed in a bag, the mobile device acting as a beacon results in a higher percent of messages picked-up \emph{correctly} near the door (46\%) than when the phone acts as a receiver (only 3\%). However, when the door is open, a higher percent of messages ``leak'' \emph{incorrectly} in mobile beacon configuration than in a mobile receiver configuration (27\% vs. 8\%). We discuss this trade-off later. 

==> Inaudible audio IUI/implementation.tex <==
\enlargethispage{\baselineskip}

\section{Augmented Proximity and Location Detection}

Our system uses ultrasonic audio beacons to augment RF-based smart applications. With standard RF-based systems, mobile devices can communicate identifying information to fixed base stations. Once the mobile application receives an RF UUID that matches a known UUID, it generates an ultrasonic message. This message can be static, globally unique, or can incorporate details of the application context, such as the RF UUID or session information. The mobile then sends this ultrasonic (US) message continuously. When the fixed receiver detects an RF signal but no US signal from the mobile beacon, it can infer that the mobile device is on the other side of a threshold. The fixed beacon can relay this information to external services (e.g., a smart door service). Once the fixed receiver detects both the RF signal and the US signal, it can infer that the mobile device is inside the space and again relay this information to external services (e.g., to lock the  door). 

Note that if there are multiple mobile devices in a space, they will all be sending ultrasonic signals to the fixed receiver. To avoid interference, mobile devices can broadcast messages on different frequency channels. The fixed device can assign open channels to each mobile device as they move within RF-range. 

Furthermore, any device with a speaker and microphone can serve as either an ultrasonic beacon or a receiver. Therefore, in the scenario describe above, the fixed device could \emph{send} ultrasonic messages and the mobile device could \emph{receive} them (Figure \ref{fig:system}). Since in that case there is only one device transmitting messages (the fixed device) this approach mitigates the need for multi-channel support. On the other hand, it makes the mobile device responsible for determining the user's location.

Finally, it is also possible to completely remove the reliance on RF-based signals. To support that case, a second ultrasonic beacon can be placed on the outside of a threshold. When the mobile device comes within range of the exterior ultrasonic device, the system can communicate to external services that the user is nearby but outside (e.g., to open a smart door). When the user is inside with the door closed, the system will detect ultrasonic signals at the interior fixed receiver but not the exterior fixed receiver, indicating that the user is inside (e.g., to lock the door).

\begin{figure}[tb]
\centering
\begin{tabular}{c} 
%\includegraphics[width=3in]{figs/system3a.png} \\
%(a) \\
\includegraphics[width=3in]{figs/system_3b_aligned.png} \\
(a) \\
\includegraphics[width=3in]{figs/system_3c_aligned.png} \\
(b) \\
\end{tabular}
\caption{Mobile and fixed devices communicate through RF and ultrasonics (US). (a) The beaconing device (here, the fixed device) then begins emitting ultrasonic messages, which cannot cross thresholds (such as doors or walls). (b) When the fixed and mobile devices are in the same space, the listening device receives ultrasonic messages and can communicate verified presence in the space to external services.}
\label{fig:system}
\end{figure}

\subsection{Implementation}
A number of tools and frameworks are available for making the development of ultrasonic-based applications simpler (cf., \cite{lee_chirp_2015,tung_cross-platform_2018,wang_messages_2016}).
In our proof-of-concept implementation, we use the Chirp SDK, an open-source framework for sending and receiving audible and inaudible audio with any desktop or mobile device \cite{chirp}. This flexibility allows us to export the system to any device with a microphone and/or a speaker. Also, the system requires no network connection and therefore can work in areas or situations that have no internet connectivity. We have also tested the system in the context of a standard teleconference meeting as well as background music in a cafe setting. In neither case was performance effected. 

Currently, beacons send short messages (two arbitrary hexadecimal characters) and use a delay to detect absence. However, we have successfully tested messages up to 16 hex characters (8 bytes) in length. It is therefore possible to generate keys specific to each application context, which can prevent against potential man-in-the-middle attacks.

% I would love to get an answer from Chrip about available channels

%\begin{figure}[htb]
%\centering
%\begin{tabular}{m{1.35in}m{.8in}m{1.45in}}
%State & Mobile device & Displays \\
%\hline
%Session active, user is away from both IAX beacons & %\includegraphics[width=.6in]{figs/mobileAwaySessionOn.png} &
%\includegraphics[width=1.25in]{figs/publicDisplayDoorLocked.png} \\
%Session active, user's device detects outside IAX beacon (only) & \includegraphics[width=.6in]{figs/mobileOutsideSessionOn.png} &
%\includegraphics[width=1.25in]{figs/publicDisplayDoorUnlocked.png} \\
%Session active,  user's device detects inside IAX beacon (only) & \includegraphics[width=.6in]{figs/mobileInsideSessionOn.png} &
%\includegraphics[width=1.25in]{figs/publicDisplayDoorLocked.png} \\
%Session inactive,  user's device detects inside IAX beacon (only) & \includegraphics[width=.6in]{figs/mobileInsideSessionOff.png} &
%\includegraphics[width=1.25in]{figs/publicDisplayDoorUnlocked.png} \\
%Session inactive,  user's device detects outside IAX beacon (only) & \includegraphics[width=.6in]{figs/mobileOutsideSessionOff.png} &
%\includegraphics[width=1.25in]{figs/publicDisplayDoorLocked.png} \\
%Session inactive,  user is away from both IAX beacons & \includegraphics[width=.6in]{figs/mobileAwaySessionOff.png} &
%\includegraphics[width=1.25in]{figs/publicDisplayDoorLocked.png} \\
%\end{tabular}
%\caption{Mobile device and public display transition states}
%\label{fig:states}
%\end{figure}

%\begin{figure}[H]
%\centering
%\includegraphics[width=4in]{figs/dataFlow.png} 
%\caption{System state settings (note that system defaults to the locked state)}
%\label{fig:dataFlow}
%\end{figure}


==> Inaudible audio IUI/intro.tex <==
\section{Introduction}
Indoor localization and proximity detection are key ingredients for many intelligent applications, services, and smart connected devices. Significant progress has been made in the accuracy and performance of wireless, radio-frequency-based (RF-based) localization solutions, using, for example, GSM \cite{otsason_accurate_2005}, Wi-Fi \cite{bahl_radar:_2000,chintalapudi_indoor_2010,biehl_loco:_2014,li_indotrack:_2017,sugasaki_robust_2017,soltanaghaei_multipath_2018}, UWB \cite{correal_uwb_2003}, Zigbee \cite{sugano_indoor_2006}, and different combinations \cite{cooper_loco:_2016} (for surveys, see \cite{liu_survey_2007,mainetti_survey_2014}). However, despite many advancements, it is still difficult for most RF-based solutions to determine if a tracked device or user is on one side of a wall or door or the other. Even past work that combines RF and inaudible audio tends to work poorly near threshold boundaries (see Figure 9 in \cite{Sosa-Sesma}). This is because the physical distance between standing on one side or another of a physical threshold is well within the accuracy limits of most localization systems. 

Consider, for example, a smart lock that cannot tell for certain whether a user is inside or outside their home, or a private document-delivery service that cannot ascertain that the user is within the designated location or not in the adjacent office.
% Consider, for example, a smart lock that can automatically unlock the door for a user when approached with a known smartphone, but must not unlock the door when the user is inside the house. Or a private document that can only be delivered when the user enters their office, but should not be sent when the user is standing in an adjacent office. 
We propose a simple yet valuable approach for overcoming this challenge by augmenting RF-based localization and proximity-detection with active audio sensing. We focus on \emph{inaudible audio}: sound waves just above 20kHz, which are beyond typical human hearing range \cite{rosen} but that are still within range of commodity microphones. Unlike RF, physical barriers, such as a closed door or walls, more strongly attenuate sound waves, making them particularly useful for threshold-detection. 

In this paper, we present a solution that relies on broadcasting and listening for ultrasonic phrases to allow an indoor-location or proximity-detection system to determine on which side of a threshold a user's device is located. We describe two potential configurations for our solution, each with different technical and privacy characteristics, and present results from an evaluation of our solution under different conditions. Specifically, this paper makes the following contributions: 1) A simple and cost-effective solution to determining position around a threshold; 2) Results from a series of tests that validate the approach but also reveal that application needs as well as the method of carrying a mobile device can have surprising impacts on optimal system configuration, and 3) a discussion of performance as well as privacy trade-offs for this use of acoustic sensing.

% \begin{figure}[tb]
% \centering
% \begin{tabular}{c} 
% \includegraphics[width=1.0\columnwidth]{figs/audio2.png} \\
% \end{tabular}
% \caption{(left) A personal workbooth with no proximity sensing. (center) Audio waves more-or-less respect threshold boundaries, allowing a system to determine whether a tracked device is (1) inside a workbooth, (2) outside the workbooth, or (3) far away from the workbooth. (right) Electromagnetic waves, while much more effective for proximity detection in general, can struggle with differentiating positions near boundaries, such as (1) and (2).}
% \label{fig:waves}
% \end{figure}

% Despite recent advances in wireless proximity-sensing technologies, it can be difficult to determine if a tracked device or user is on one side of a wall or door or the other. This difficulty arises from the fact that the difference in actual distance between outside and inside a space is often less than a foot, which is well within the margin of error of tracking systems that depend on estimated distance based on relative received signal strength (RSSI) of electromagnetic field (EMF) waves (e.g., WiFi, GPS, Bluetooth, etc.).
% For example, current Smart Locks \cite{august,fridaylabs,ottoCNET,danalock} will offer Geofencing to unlock the door when a user's device is in proximity of the lock and automatically unlock the door when the user is far from the lock. However, in order to avoid automatically unlocking the door when the user is inside, these locks will typically rely on several assumptions  (e.g., that the user went inside after opening the door) that can lead to errors (e.g., the user could have stayed outside, but the system assumes they are no inside and avoid unlocking the door).
% In some environments, these technologies are therefore combined with motion senors, NFC or other very near-field technologies to determine actual presence in a space. However, motion sensors cannot attribute presence to a particular individual (or device) and near-field technologies require users to actively badge in to a room, which can be cumbersome or produce state errors if the user forgets to badge out.

% Contrary to EMF waves, sound waves are more likely to respect wall and door boundaries and therefore can be more useful for threshold boundary scenarios (Figures \ref{fig:waves} and \ref{fig:waves2}). Furthermore, unlike NFCs, they do not require any specific user actions. They can also send a small amount of data over short distances, providing extra information at a short range, which is not possible with NFC.

% At frequencies above 20Khz, sound waves are inaudible to the human ear but can still be picked up by commodity microphones. Sound waves at those frequencies can be referred to as inaudible audio. (Studies report that ultrasounds above 22Khz seem inaudible as long as their level does not exceed 85dB \cite{ashihara_audibility_2000}.)

% In this work we propose to utilize inaudible audio beacons to reliably detect a user device's presence on one side or the other of a physical threshold (i.e., a door). We combine our solution with an external scheduling system to determine whether the door should be locked or unlocked for a particular user at a given time. We can also optionally combine inaudible audio beacons with EMF-based proximity services.

% \begin{figure}[tb]
% \centering
% \begin{tabular}{c} 
% \includegraphics[width=1.0\columnwidth]{figs/audio3.png} \\
% \end{tabular}
% \caption{(left) When two workbooths are positioned next to each other it can be difficult to determine which user is in which booth with electromagnetic wave-based approaches. (right) Using ultrasonics, this is not an issue.}
% \label{fig:waves2}
% \end{figure}

% \begin{figure}[tb]
% \centering
% \begin{tabular}{c} 
% \includegraphics[width=2in]{figs/audio4.png} \\
% \end{tabular}
% \caption{An interior ultrasonic sensor can be combined with a Bluetooth sensor to determine that a user is generally in the area and that a user is inside or outside of a particular space.}
% \label{fig:waves3}
% \end{figure}




==> Inaudible audio IUI/related_work.tex <==
\section{Related work}
A growing body of work has demonstrated the broad appeal of acoustic sensing as a low cost and ubiquitous approach for spatial interaction \cite{gupta_soundwave:_2012,aumi_doplink:_2013, watanabe_ultrasound-based_2013,laput_sweepsense:_2016,nishida_real_2004,zhang_soundtrak:_2017}, context-aware applications \cite{li_condiosense:_2017}, localization \cite{rossi_roomsense:_2013,tarzia_indoor_2011,azizyan_surroundsense:_2009,schweinzer_ultrasonic_2010,lazik_indoor_2012,mao_cat:_2016,qiu_silent_2017}, and device-to-device communication and interaction \cite{lee_chirp_2015,tung_cross-platform_2018,wang_messages_2016,Jin2015}. However, many of these systems require extensive infrastructure, which can be difficult to deploy and maintain \cite{Ward}. Other work mentions threshold detection (for automobiles) only as future work \cite{laput_sweepsense:_2016}.

In the area of indoor localization, passive acoustic sensing can be used to match fingerprints of ambient audio captured in different spaces \cite{azizyan_surroundsense:_2009,rossi_roomsense:_2013,tarzia_indoor_2011}. One potentially limiting assumption with this approach is that spaces must be sufficiently acoustically different. With active acoustic sensing-based localization, audio is emitted and captured by the user's device or speakers in the environment \cite{schweinzer_ultrasonic_2010,lazik_indoor_2012,mao_cat:_2016,qiu_silent_2017}. Mao \textit{et al.}, for example, use an array of ultrasonic speakers within a room to perform accurate 3D spatial localization \cite{mao_cat:_2016}. 

For the task of determining what side of a threshold or wall a user is standing, prior research also explored several non-acoustic approaches. For example, sensing changes in air-pressure when people move between rooms or close doors \cite{patel_detecting_2008}, or by using a radar mounted above the doorway and categorizing users by their body shape \cite{kalyanaraman_forma_2017}. Others use knowledge of walls within the space from map data to improve non-acoustic predicted localization (\textit{c.f.}, \cite{li_reliable_2012,lazik_indoor_2012,biswas_wifi_2010}). Our approach, which we describe next, relies on active acoustic sensing as a cost-effective solution for augmenting RF-based localization or proximity-detection systems.

==> applications_leftovers.tex <==
% \subsection{Telemedicine kiosks}
% Most doctor visits are fast, taking only on average ~17 minutes \footnote{https://www.ncbi.nlm.nih.gov/pmc/articles/PMC2254573/}. However, it can be important for a doctor to have some basic information about a patient's medical history, such as test results or past and current prescriptions, before making a diagnosis. For visits at a traditional doctor's office, obtaining this information securely is straightforward. However, at a telemedicine kiosk this information would need to be sent from a patient through a wireless network, and nearby malingerers could intercept the data. Information could be encrypted on the user's mobile device, but in some cases that may take too long or be impractical. Sending information back-and-forth from the patient to the booth via ultrasonic communication, then relying on the booth system to encrypt and send the data to the doctor over a wired network, could provide a high level of security and privacy without forcing users to worry about encrypting their data.

% \subsection{Room-based music differentiation}
% While homes and workspaces often share a common music service (e.g., Sonos), people may want to play different music in different rooms or office spaces. While this is technically possible with such systems, since they have no method of determining the room a user is currently in, the process is complicated \footnote{ https://drive.google.com/file/d/1mI9AOixsZpxDrxVnsnzYQbPZ23bSV-EG/view}. Furthermore, these systems can be trivially hacked so that users in one part of the house or office play unwanted music in a different part of the house or office. 

% On the other hand, using a combination of mobile devices and IAX beacons, the system can be configured to play music in the current room and only the current room with a single button press. Furthermore, since IAX beacons can be any device with a speaker, an Alexa (or similar) device can be re-purposed as an IAX beacon. 

% \subsection{Conference presentations}

% \begin{figure}[htb]
% \centering
% \begin{tabular}{cc} 
% \includegraphics[width=1.5in]{figs/confUI1.png} & \includegraphics[width=1.5in]{figs/confUI2.png}\\
% \end{tabular}
% \caption{At many conferences, attendees can take advantage of mobile apps that provide special services for talks. Without IAX beacons (left), users must manually find the room they are currently in. With IAX beacons (right), their device can automatically find their current room and allow them to access services directly.}
% \label{fig:conference}
% \end{figure}

% Increasingly, conferences offer extra services to audience members, such as slides of the current talk or a backchannel chat or translation services \cite{lanbridge}. While, again, using Bluetooth or other EMF-based technologies would make it possible to select the current talk amongst a list, in large conferences with many simultaneous talks it would be difficult to find the one occurring in the room the user is in. On the other hand, using ultrasonic audio, the user can can connect directly to the talk happening in their room. Furthermore, speakers could include interactive sections of their talk, including live polling or feedback solicitation, and be confident that only those audience members currently in the room would be able to participate.

% In some environments, these technologies are therefore combined with motion senors, NFC or other very near-field technologies to determine actual presence in a space. However, motion sensors cannot attribute presence to a particular individual (or device) and near-field technologies require users to actively badge in to a room, which can be cumbersome or produce state errors if the user forgets to badge out.

% Our combined RF- and ultrasonic-based approach, on the other hand, can reduce or eliminate these ambiguities without requiring the user to take any explicit action. In this case, the Smart Lock would act as the receiver, listening to ultrasonic messages sent from the mobile on the inside of the door. Once it receiving messages from the interior ultrasonic sensor, and the door is shut, it can safely assume that the user is inside and lock the door.

% Contrary to EMF waves, sound waves are more likely to respect wall and door boundaries and therefore can be more useful for threshold boundary scenarios (Figures \ref{fig:waves} and \ref{fig:waves2}). Furthermore, unlike NFCs, they do not require any specific user actions. They can also send a small amount of data over short distances, providing extra information at a short range, which is not possible with NFC.

% Private workbooths, such as Jabbrrbox \cite{jabbrrbox}, that are placed in public areas rely on automatic access systems that our RF- and ultrasonic-based approach can augment. Here again, the system can use an RF sensor coupled with an internal ultrasonic receiver to determine whether the user is outside or inside the workbooth. Furthermore, the system can connect to an external service that indicates whether the user currently has access to a nearby workbooth, allowing the system to determine the following several states. 

%\begin{figure}[tb]
%\centering
%\includegraphics[width=2in]{figs/jabbrrbox.jpg} 
%\caption{The Jabbrbox workbooth  \cite{jabbrrbox}.}
%\label{fig:jabbrrbox}
%\end{figure}

% \textbf{Session active, user is away from both the RF and US beacons:} The system notifies the user to proceed to the workbooth. 

% \textbf{Session active, the workbooth detects that the user is in RF range (only):} The system unlocks the door for the user.

% \textbf{Session active, the workbooth detects that the user in US range and the door is shut:} The system locks the workbooth. 

% \textbf{Session inactive, the workbooth detects that the user in US range:} The system unlocks the door for the user and notifies the user that their session is over. 

% \textbf{Session inactive, the workbooth detects that the user is not in US range:} The system takes no action. 

% The default case is that the system will remain locked. 

% One additional useful case is when several workbooths are located next to one another in the same space. In this case, the system can broadcast encrypted, identifying messages on unique RF and US channels to provide the user access only to the workbooth they have scheduled.



==> eval_leftovers.tex <==


% \paragraph{Inaudible audio is secure} In all cases in which the door was shut and the user location was different from the fixed device location (1040 total samples), zero messages were transferred. This implies that if a user is outside of a room with the door shut the system will never erroneously register a user as inside a room. However, in further experimentation, we found that this is only true if the door is well insulated (that is, a user holding a device right next to a poorly insulated closed door may be able to send messages to an interior fixed device). 

% \paragraph{Message sending works well when the device is unimpeded but degrades rapidly} When the user is on the same side as the fixture location and holding the device in their hand, message sending works well (320/320 received in the near condition, 311/320 received in the far condition). Also, a relatively high percentage of messages are received when the device is in a user's pocket (301/320 received in the near condition, 178/320 received in the far condition). However, far fewer messages are received when the device is placed in a bag (79/320 received in the near condition, 9/320 received in the far condition). While not surprising, this result does imply that users who tend to carry their device in a bag or purse will need to take it out or rely a smartwatch. 

% \paragraph{Messages sent from the mobile are more likely to be received than those sent from a fixed device} More messages are transferred when the mobile device is the one sending data (814/1920 events received by the fixed device) than the reverse (555/1920 events received by the mobile). This is especially true when the mobile device is in a bag and sending (82/640 events received at the fixed location) versus receiving (6/640 events received by the mobile). This implies that the device's microphone suffers more attenuation than does its speaker.

% \paragraph{It is possible to detect when the door is open in some cases} When the user is on the opposite side from the fixed device, near the threshold, and the user is holding the device in their hand, the system can potentially detect that the door is open (107/320 events received) versus shut (0/320 events received). However, if the device is in a user's pocket, the difference between open (41/320 events received) and shut (0/320 events received) is smaller. The difference between the door being open and shut is not detectable when the device is in a bag (0/320 for both cases).

%\colorbox{pink}{highlight}

%%To better understand the performance of our solution under a range of conditions, we carried a set of experiments.

%%We compared:

%%Door type
%%Indoor vs. Outdoor performance
%%Mobile device location (in hand vs. pocket vs. purse)

%%We tested each combination at four positions as illustrated in Figure XXX; two positions outside and two positions inside. We further tested each combination with the door open and with the door shut.

%%Test devices:  Android? Google Pixel vX?
%%Based on a pilot test, transmission volume in all tests was set to XXX. 

%%In each test case, the system transmitted the phrase 20 times. Our recognition results are presented as a percent of phrases picked up correctly by the receiving device.
